ShareGPT4Video: Improving Video Understanding and Generation with Better Captions

We present the ShareGPT4Video series, aiming to facilitate the video understanding of large video-language models (LVLMs) and the video generation of text-to-video models (T2VMs) via dense and precise captions. The series comprises: 1) ShareGPT4Video, 40K GPT4V annotated dense captions of videos with various lengths and sources, developed through carefully designed data filtering and annotating strategy. 2) ShareCaptioner-Video, an efficient and capable captioning model for arbitrary videos, with 4.8M high-quality aesthetic videos annotated by it. 3) ShareGPT4Video-8B, a simple yet superb LVLM that reached SOTA performance on three advancing video benchmarks. To achieve this, taking aside the non-scalable costly human annotators, we find using GPT4V to caption video with a naive multi-frame or frame-concatenation input strategy leads to less detailed and sometimes temporal-confused results. We argue the challenge of designing a high-quality video captioning strategy lies in three aspects: 1) Inter-frame precise temporal change understanding. 2) Intra-frame detailed content description. 3) Frame-number scalability for arbitrary-length videos. To this end, we meticulously designed a differential video captioning strategy, which is stable, scalable, and efficient for generating captions for videos with arbitrary resolution, aspect ratios, and length. Based on it, we construct ShareGPT4Video, which contains 40K high-quality videos spanning a wide range of categories, and the resulting captions encompass rich world knowledge, object attributes, camera movements, and crucially, detailed and precise temporal descriptions of events. Based on ShareGPT4Video, we further develop ShareCaptioner-Video, a superior captioner capable of efficiently generating high-quality captions for arbitrary videos...

==> backup.tex <==

\subsection{Experimental Setup}

% \textbf{Datasets.} For the video understanding task, the primary goal is to validate that the high-quality video-caption data collected in ShareGPT4Video can effectively enhance various LVLMs' performance in comprehending the wild world comprehensively. To achieve this, we integrate 28K high-quality video-caption data related to complex scenes (Panda-70M \cite{chen2024panda}, Ego4D \cite{grauman2022ego4d}, and BDD100K \cite{yu2020bdd100k}) collected from ShareGPT4Video either by (1) replacing low-quality video-caption data in the current training data, or (2) combining them with existing instructional VQA data. In the first scenario, we opt to replace the captions data in the VideoChatGPT-100K \cite{maaz2023video} conversation data with an equivalent number of 28K high-quality captions sourced from ShareGPT4Video. In the second scenario, we first collect 153K VQA data from various instructional video-to-text datasets to build our baseline. This collection includes 13K conversational data from VideoChatGPT \cite{maaz2023video} and 140K question-answer pairs, with 45K data points from CLEVRER \cite{yi2019clevrer}, 8K from EGO-QA \cite{grauman2022ego4d}, 34K from NextQA \cite{xiao2021next}, and 53K from TGIF-Transition \cite{li2016tgif}. Then, these VQA data are combined with 28K video-caption data, forming a consolidated training dataset of 181K samples. 



\textbf{Implementation Details.} We utilize GPT-4-Turbo-04-09 for generating high-quality captions. When validating the effectiveness of our high-quality video-caption data on existing LVLMs, such as VideoLLaVA \cite{lin2023video} and LLaMA-VID \cite{li2023llama}, all training settings and hyperparameters are kept unchanged to isolate the impact of the improved captions. To verify that high-quality video-caption data can be combined with VQA data to enhance LVLM further and to obtain our final ShareGPT4Video-8B model, we start with the LLaVA-Next-8B \cite{li2024llavanext-strong} image multi-modal model. Consistent with previous LVLM approaches \cite{lin2023video,maaz2023video}, we uniformly sample 16 frames from each video and arrange these frames into a 4x4 image grid to form the input for both training and inference, following the IG-VLM \cite{kim2024image} strategy. During training, we employ a batch size of 128 and the AdamW optimizer. We opt to fine-tune the entire model, setting the learning rate for the vision encoder at 2e-6, for the MLP projector at 2e-5, and for the LLM using LoRA \cite{hu2021lora}, the learning rate is set at 2e-4. Such training strategy enables us to obtain an exceptional LVLM, ShareGPT4Video-8B, with \textbf{8 A100 GPUs in about 5 hours}. To validate the effectiveness of high-quality captions in the T2VMs area, we utilize ShareCaptioner-Video and Panda-Student \cite{chen2024panda} to generate high-quality and short video captions for 4.5M videos with 65 frames and 0.3M videos with 221 frames, separately. Following the process outlined in the Open-Sora-Plan \cite{pku_yuan_lab_and_tuzhan_ai_etc_2024_10948109}, we fine-tuned the pretrained T2VM to enable the generation of high-fidelity 10-second videos.

% \subsection{Caption quality analysis}

% \textbf{Qualitative captioning capability comparison between ShareCaptioner-Video and GPT4V.} We first analyze the linguistic composition of the captions produced by GPT4V and ShareCaptioner-Video, and the results are presented in Figure 5. The analysis reveals that the captions generated by our ShareCaptioner-Video contain a comparable information level to those generated by GPT4V. Furthermore, as shown in Figure 7, we first generate 100 captions with GPT4V and ShareCaptioner-Video and then invite 10 volunteers to evaluate the captions based on three aspects. These aspects include (1) \textbf{Omission and Fabrication} - checking for no key elements missing in the caption and identifying imaged elements not present in the video; (2) \textbf{Distortion} - assessing the accuracy of element attributes such as color and size; and (3) \textbf{Temporal Mismatch} - evaluating whether the description accurately reflects the evolution of temporal events in the video. Each pair can earn a maximum of 3 points, one for each criterion met. As anticipated, our ShareCaptioner-Video performs on par with the GPT4V.

\subsection{Main Results for Video Understanding}

\textbf{Effectiveness of ShareGPT4Video Dataset.} We validated the effectiveness of ShareGPT4Video in enhancing video comprehension capabilities under two data settings. In the first setting, we utilize a video-caption subset with 28K high-quality samples from ShareGPT4Video to replace an equivalent portion of the 100K video instruction tuning data \cite{maaz2023video} used in current LVLMs \cite{lin2023video,li2023llama}. As shown in Table \ref{tab:ablation1}, ShareGPT4Video consistently improves the alignment between video and language modalities in different LVLM architectures and scales. Specifically, VideoLLaVA-7B \cite{lin2023video} achieves an average performance gain of 1.1 across three comprehensive multi-modal video benchmarks after integrating high-quality captions, while LLaMA-VID-7B and LLaMA-VID-13B achieve an average gain of 2.0 and 2.3, separately. Our high-quality video-caption data is particularly effective in helping LVLMs achieve significant performance improvements on benchmarks that require complex temporal understanding, such as TempCompass \cite{liu2024tempcompass}. In the second setting, we combine the newly collected VQA data with an equal amount of either short captions from Panda-70M \cite{chen2024panda} or detailed captions from our ShareGPT4Video. The baseline involves using the collected 153K VQA data and adapting the LLaVA-Next-8B \cite{liu2024llavanext} image multimodal model into a video multimodal model using the IG-VLM \cite{kim2024image} strategy. As indicated in Table \ref{tab:ablation2}, introducing short captions on top of VQA data may not yield substantial performance gains. It could even degrade performance on some benchmarks due to sub-optimal modality alignment. Comparing the first, second, and fourth rows of Table \ref{tab:ablation2}, the significant performance gains of comprehending temporal sequences benefited from our high-quality caption data are evident. Moreover, unlocking the vision encoder when training with detailed captions facilitates better modality alignment for LVLMs.



\textbf{Quantitative Comparison of LVLMs.} As illustrated in Table \ref{tab:tempcompass}, \ref{tab:vbench}, \ref{tab:mvbench}, we present a quantitative comparison between our ShareGPT4Video-8B model supercharged by our ShareGPT4Video dataset with existing state-of-the-art LVLMs. Notably, compared with previous LVLMs, our ShareGPT4Video-8B attains the most superior performance in all three comprehensive benchmarks. 
% Specifically, on the TempCompass benchmark, previous LVLMs could easily achieve higher scores in the Action category, while lacking capabilities in the remaining categories of perception speed, direction, event sequence, and attribute changes. This discrepancy arises because actions can largely be inferred from static visual cues, whereas the other four categories rely more heavily on a deep understanding of temporal information between frames. 
Specifically, thanks to the rich temporal information provided by ShareGPT4Video, our ShareGPT4Video-8B model achieves an impressive average accuracy of 61.5\% on the TempCompass benchmark. This is an 11.6\% increase over the previous best-performing LVLM, VideoLLaVA-7B.
% Thanks to the rich temporal information provided by ShareGPT4Video, our ShareGPT4Video-8B model achieved the best scores in 19 out of 20 dimensions, with an impressive average accuracy of 61.5\%. This is an 11.6\% increase over the previous best-performing LVLM, VideoLLaVA-7B. This significant performance improvement is primarily observed in the dimensions of event sequence and attribute changes.
Additionally, despite the VideoBench and MVBench benchmarks collecting a diverse range of QA data from various existing video datasets, we achieve solid performance on these benchmarks, surpassing the previous state-of-the-art by an average accuracy of 2.7\% and 8.2\%, respectively.
% Notably, on MVBench, our model secures either first or second place in 15 out of the 20 evaluation dimensions.



==> figures/captioner-statistics.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/files/captioner-statistics.pdf}
    \captionsetup{font={footnotesize}}
    \caption{Dataset Statistics}
    \label{fig:captioner}
\end{figure*}

==> figures/key_frame_code.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/files/key_frame_code.pdf}
    \captionsetup{font={footnotesize}}
    \caption{Pseudo code for semantic-aware key-frame extraction.}
    \label{fig:key_frame_code}
\end{figure*}

==> figures/pseudo_code.tex <==
\begin{figure}[!t]
    \centering
    \begin{minipage}[h]{0.49\textwidth}
        \centering
        \captionsetup{font={scriptsize}}
        \vspace{-11.5pt}
        \resizebox{\textwidth}{!}{
        \includegraphics[width=0.99\linewidth]{figures/files/bert.pdf}
        }
        \captionof{figure}{Pseudo code of semantic-based data filtering.}
        \label{fig:code1}
    \end{minipage}
    \quad
    \begin{minipage}[h]{0.47\textwidth}
        \centering
        \captionsetup{font={scriptsize}}
        \vspace{-11.5pt}
        \resizebox{\textwidth}{!}{
        \includegraphics[width=0.99\linewidth]{figures/files/key_frame_code.pdf}
        }
        \captionof{figure}{Pseudo code of semantic-aware key-frame extraction.}
        \label{fig:code2}
    \end{minipage}
\end{figure}

==> tables/lvlm_all.tex <==
\begin{table*}[!t]
    \setlength\tabcolsep{4pt}
    \centering
    \footnotesize
    \captionsetup{font={footnotesize}}
    \caption {\textbf{Comparison with SOTA methods on three video multi-modal benchmarks.} With 7B parameters, ShareGPT4Video-8B outperforms competitors in all three benchmarks, despite these competitors using larger training data or more parameters. The best results are \textbf{bold} and the second-best results are \underline{underlined}.}\label{tab:lvlm_all}
    % \vspace{-2mm}
	% \captionsetup[subfloat]{}
	\captionsetup[subffloat]{justification=centering}
    \subfloat[TempCompass \cite{liu2024tempcompass}\label{tab:temp}]{
        \renewcommand{\arraystretch}{1.25}
		\resizebox{0.3\textwidth}{!}{
        \begin{tabular}{l|c}
            \toprule
            Model             & Avg.          \\ \midrule
            Valley-7B \cite{luo2023valley}         & 33.4          \\
            PandaGPT-13B \cite{chen2024panda}      & 40.4          \\
            VideoLLaMA-13B \cite{zhang2023video}    & 43.3          \\
            VideoChatGPT-7B \cite{maaz2023video}   & 42.4          \\
            mPLUG-Owl-7B \cite{ye2023mplug}      & 44.5          \\
            VideoLLaVA-7B \cite{lin2023video}     & {\ul 49.9}          \\
            LLaMA-VID-7B \cite{li2023llama}      & 44.2          \\ \midrule
            ShareGPT4Video-8B & \textbf{61.5} \\ \bottomrule
        \end{tabular}
        }
    }
    \hspace{0.5mm}
    \subfloat[VideoBench \cite{ning2023video}\label{tab:vbench}]{
        \renewcommand{\arraystretch}{1.15}
		\resizebox{0.25\textwidth}{!}{
        \begin{tabular}{l|c}
            \toprule
            Model             & Avg.          \\ \midrule
            mPLUG-Owl-7B \cite{ye2023mplug}         & 33.2          \\
            Otter-7B \cite{li2023otter}      & 37.5          \\
            VideoLLaMA-7B \cite{zhang2023video}    & 32.8          \\
            Valley-7B \cite{luo2023valley}   & 34.0          \\
            VideoChat-7B \cite{li2023videochat}      & 35.4          \\
            PandaGPT-7B \cite{chen2024panda}     & 37.5          \\
            VideoChatGPT-7B \cite{maaz2023video}      & {\ul 38.5}    \\
            ChatUniVi-7B \cite{jin2023chat}      & 35.3    \\
            VideoLLaVA-7B \cite{lin2023video}      & 34.5    \\
            LLaMA-VID-7B \cite{li2023llama}      & 36.5    \\
            \midrule
            ShareGPT4Video-8B & \textbf{41.2} \\ \bottomrule
        \end{tabular}
        }
    }
    \hspace{0.5mm}
    \subfloat[MVBench \cite{li2023mvbench}\label{tab:mvbench}]{
        \renewcommand{\arraystretch}{1.15}
		\resizebox{0.295\textwidth}{!}{
        \begin{tabular}{l|c}
            \toprule
            Model             & Avg.          \\ \midrule
            Otter-7B \cite{li2023otter}        & 26.8          \\
            mPLUG-Owl-7B \cite{ye2023mplug}      & 29.7          \\
            LLaMA-Adapter \cite{zhang2023llama}    & 31.7          \\
            VideoChatGPT-7B \cite{maaz2023video}   & 32.7          \\
            VideoLLaMA-7B \cite{zhang2023video}      & 34.1         \\
            VideoChat-7B \cite{li2023videochat}     & 35.5          \\
            VideoLLaVA-7B \cite{lin2023video}      & {\ul 43.0}    \\
            LLaMA-VID-7B \cite{li2023llama}      & 41.3    \\ \midrule
            ShareGPT4Video-8B & \textbf{51.2} \\ \bottomrule
        \end{tabular}
        }
    }
\end{table*}
